Formal guarantees for heuristic optimization algorithms used in machine learning

Recently, Stochastic Gradient Descent (SGD) and its variants have become the dominant methods in the large-scale optimization of machine learning (ML) problems. A variety of strategies have been proposed for tuning the step sizes, ranging from adaptive step sizes to heuristic methods to change the step size in each iteration. Also, momentum has been widely employed in ML tasks to accelerate the training process. Yet, there is a gap in our theoretical understanding of them. In this work, we start to close this gap by providing formal guarantees to a few heuristic optimization methods and proposing improved algorithms. First, we analyze a generalized version of the AdaGrad (Delayed AdaGrad) step sizes in both convex and non-convex settings, showing that these step sizes allow the algorithms to automatically adapt to the level of noise of the stochastic gradients. We show for the first time sufficient conditions for Delayed AdaGrad to achieve almost sure convergence of the gradients to zero. Moreover, we present a high probability analysis for Delayed AdaGrad and its momentum variant in the non-convex setting. Second, we analyze SGD with exponential and cosine step sizes, which are empirically successful but lack theoretical support. We provide the very first convergence guarantees for them in the smooth and non-convex setting, with and without the Polyak-{\L}ojasiewicz (PL) condition. We also show their good property of adaptivity to noise under the PL condition. Third, we study the last iterate of momentum methods. We prove the first lower bound in the convex setting for the last iterate of SGD with constant momentum. Moreover, we investigate a class of Follow-The-Regularized-Leader-based momentum algorithms with increasing momentum and shrinking updates. We show that their last iterate has optimal convergence for unconstrained convex stochastic optimization problems.

==> 0_Prelim/cv.tex <==
\addcontentsline{toc}{chapter}{Curriculum Vitae}
%
\begin{center}
{\LARGE {\bf CURRICULUM VITAE}}\\
\vspace{0.5in}
{\large {\bf Xiaoyu Li}
\\
xyli0706@gmail.com}
\end{center}

\begin{center}
{\large {\bf Education}}
\end{center}

\begin{longtable}{p{9.5cm} p{4cm}}
%	\hline
\multicolumn{2}{c}{}\\
\textbf{Boston University}& Sep. 2018 - June 2022\\
Ph.D. in System Engineering &Boston, MA  \\
Advisor: Francesco Orabona& \\


\multicolumn{2}{c}{}\\
\textbf{Stony Brook University}& Aug. 2016 - Aug 2018\\
Ph.D. Candidate in Applied Math. \& Statistics &Stony Brook, NY  \\
Advisor: Francesco Orabona& \\

\multicolumn{2}{c}{}\\
\textbf{University of Science and Technology of China}& Aug. 2012 - June 2016\\
Bachelor in Mathematics \& Applied Mathematics &Hefei, China  \\

\end{longtable}

\begin{center}
{\large {\bf  Professional Experience}}
\end{center}
\begin{longtable}{p{9cm} p{4cm}}
%	\hline
\multicolumn{2}{c}{}\\
\textbf{Boston University}& Sep. 2018 - June 2022\\
Research Assistant &Boston, MA  \\


\multicolumn{2}{c}{}\\
\textbf{Amazon}& June 2021 - Aug 2021\\
Applied Scientist Intern & Remote \\

\multicolumn{2}{c}{}\\
\textbf{Nokia Bell Labs}& June 2019 - Aug. 2019\\
Research Summer Intern & Murray Hill, NJ \\	
\end{longtable}

\begin{center}
{\large {\bf  Publications}}
\end{center}

\begin{enumerate}
\item Xiaoyu Li, Mingrui Liu, and Francesco Orabona. \textit{On the Last Iterate Convergence of Momentum Methods.} In International Conference on Algorithmic Learning Theory, pp. 699-717. PMLR, 2022.
\item 
Xiaoyu Li, Zhenxun Zhuang, and Francesco Orabona. \textit{A second look at exponential and cosine step sizes: Simplicity, adaptivity, and performance.} In International Conference on Machine Learning, pp. 6553-6564. PMLR, 2021
\item Xiaoyu Li and Francesco Orabona. \textit{A High Probability Analysis of Adaptive SGD with Momentum.} In Workshop on Beyond First Order Methods in ML Systems at ICML'20. 2020.
\item Xiaoyu Li and Francesco Orabona. \textit{On the convergence of stochastic gradient descent with adaptive stepsizes.} In The 22nd international conference on artificial intelligence and statistics, pp. 983-992. PMLR, 2019.
\end{enumerate}

\begin{center}
{\large {\bf Professional Service}}
\end{center}

Reviewer for ICML, NeurIPS, AISTATS, ICLR and JMLR 

==> 0_Prelim/quote.tex <==
\phantom{.}
\vspace{4in}

\begin{singlespace}
\begin{quote}
  \textit{Facilis descensus Averni;}\\
  \textit{Noctes atque dies patet atri janua Ditis;}\\*
  \textit{Sed revocare gradum, superasque evadere ad auras,}\\
  \textit{Hoc opus, hic labor est.}\hfill{Virgil (from Don's thesis!)}
\end{quote}
\end{singlespace}

% \vspace{0.7in}
%
% \noindent
% [The descent to Avernus is easy; the gate of Pluto stands open night
% and day; but to retrace one's steps and return to the upper air, that
% is the toil, that the difficulty.]

